An analysis of Reinforcement Learning applied to Coach task in IEEE Very Small Size Soccer

The IEEE Very Small Size Soccer (VSSS) is a robot soccer competition in which two teams of three small robots play against each other. Traditionally, a deterministic coach agent will choose the most suitable strategy and formation for each adversary's strategy. Therefore, the role of a coach is of great importance to the game. In this sense, this paper proposes an end-to-end approach for the coaching task based on Reinforcement Learning (RL). The proposed system processes the information during the simulated matches to learn an optimal policy that chooses the current formation, depending on the opponent and game conditions. We trained two RL policies against three different teams (balanced, offensive, and heavily offensive) in a simulated environment. Our results were assessed against one of the top teams of the VSSS league, showing promising results after achieving a win/loss ratio of approximately 2.0.

==> algorithms/create_dataset.tex <==

\begin{algorithm}[!ht]

\KwIn{$N_{rows}$ // Number of rows of the dataset}
\nonl\myinput{$N_{m}$ // Number of matches with the same initial positions}
\KwResult{The supervised dataset}

$N_{rows} = N_{rows}/N_{m}$

\For{$idx = 1 \rightarrow N_{rows}$}
{
    Select random positions for the robots and ball
    
    \For{$n = 1 \rightarrow N_{m}$}
    {
    Select random behaviors for each robot
    
    Simulate the match
    
    Store the inicial positions, behaviors, and the final score of the match
    
    }

}

\caption{Creation of supervised dataset}
\label{alg:dataset}
\end{algorithm}


==> figures/demo.tex <==
   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture. This will be a pic of VSSS
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   
   


==> tables/param.tex <==
\begin{table}[thpb]
\centering
\caption{Parameters Used in this Paper }
\label{tab:param}
\resizebox{0.16\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
Parameter & Value  \\ \midrule
$N_{rows}$  & 10.000 \\
$N_m$       & 10     \\ 
$N_r$       & 3      \\ \bottomrule
\end{tabular}%
}
\end{table}
